From Commands to Goal-based Dialogs: A Roadmap to Achieve Natural Language Interaction in RoboCup@Home

On the one hand, speech is a key aspect to people's communication. On the other, it is widely acknowledged that language proficiency is related to intelligence. Therefore, intelligent robots should be able to understand, at least, people's orders within their application domain. These insights are not new in RoboCup@Home, but we lack of a long-term plan to evaluate this approach. In this paper we conduct a brief review of the achievements on automated speech recognition and natural language understanding in RoboCup@Home. Furthermore, we discuss main challenges to tackle in spoken human-robot interaction within the scope of this competition. Finally, we contribute by presenting a pipelined road map to engender research in the area of natural language understanding applied to domestic service robotics.

==> Makefile <==
PREFIX  = "From_Commands_to_Goal-based_Dialogs_-_A_Roadmap_to_Achieve_Natural_Language_Interaction_in_RoboCupAtHome"
SILENT  = @
TEXFILE = $(PREFIX).tex
PDFFILE = $(PREFIX).pdf
AUXFILE = $(PREFIX).aux
TEX     = pdflatex
TEXFOPT = -halt-on-error -draftmode
TEXOPT  = -output-format=pdf
BIB     = bibtex
BIBOPT  = 

TEMP	= *.aux *.bbl *.blg *.log *.out *.tmp *.synctex.gz
RMFILES = $(TEMP) *~ *.toc *.idx *.ilg *.ind *.log *.lot *.lof \
          *.adx *.and *.abb *.ldx .temp* *.tar mergedfile.pdf

all:
	$(SILENT) make -s build
	$(SILENT) make -s launch
# $(SILENT) make -s clean

build:
	$(SILENT) rm -f $(TEMP)
	$(SILENT) $(TEX) $(TEXFOPT) $(TEXOPT) $(TEXFILE)
	$(SILENT) $(BIB) $(AUXOPT) $(AUXFILE)
	$(SILENT) $(TEX) $(TEXOPT) $(TEXFILE)
	$(SILENT) $(TEX) $(TEXOPT) $(TEXFILE)
#	$(SILENT) rm -f $(TEMP)

clean:
	$(SILENT) rm -f img/*-converted-to.pdf
	$(SILENT) rm -f $(TEMP)

launch:
	# $(SILENT) gnome-open $(PREFIX).pdf &> /dev/null
	$(SILENT) xdg-open $(PDFFILE) &> /dev/null

